Kernel-Based Structural Equation Models for Topology Identification of Directed Networks

Structural equation models (SEMs) have been widely adopted for inference of causal interactions in complex networks. Recent examples include unveiling topologies of hidden causal networks over which processes such as spreading diseases, or rumors propagate. The appeal of SEMs in these settings stems from their simplicity and tractability, since they typically assume linear dependencies among observable variables. Acknowledging the limitations inherent to adopting linear models, the present paper advocates nonlinear SEMs, which account for (possible) nonlinear dependencies among network nodes. The advocated approach leverages kernels as a powerful encompassing framework for nonlinear modeling, and an efficient estimator with affordable tradeoffs is put forth. Interestingly, pursuit of the novel kernel-based approach yields a convex regularized estimator that promotes edge sparsity, and is amenable to proximal-splitting optimization methods. To this end, solvers with complementary merits are developed by leveraging the alternating direction method of multipliers, and proximal gradient iterations. Experiments conducted on simulated data demonstrate that the novel approach outperforms linear SEMs with respect to edge detection errors. Furthermore, tests on a real gene expression dataset unveil interesting new edges that were not revealed by linear SEMs, which could shed more light on regulatory behavior of human genes.

==> mysymbol.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%theorem environments
%


\newtheorem{assumption}{\hspace{0pt}\bf AS\hspace{-0.15cm}}

\newcounter{lemma} \setcounter{lemma}{1}
\newenvironment{lemma}{ \vspace{-0.1cm} \noindent {\bf Lemma
\thelemma :} \addtocounter{lemma}{-1}\refstepcounter{lemma} \em} {\addtocounter{lemma}{1}
\vspace{-0.1cm} \normalfont }

\newcounter{corollary} \setcounter{corollary}{1}
\newenvironment{corollary}{ \vspace{-0.1cm} \noindent {\bf Corollary
\thecorollary :} \addtocounter{corollary}{-1}\refstepcounter{corollary} \em} {\addtocounter{corollary}{1}
\vspace{-0.1cm} \normalfont }

\newcounter{proposition} \setcounter{proposition}{1}
\newenvironment{proposition}{ \vspace{-0.1cm} \noindent {\bf Proposition
\theproposition :} \addtocounter{proposition}{-1}\refstepcounter{proposition}\em } { \addtocounter{proposition}{1}
\vspace{-0.1cm} \normalfont }

\newtheorem{observation}{\hspace{0pt}\bf Observation}
\newtheorem{theorem}{\hspace{0pt}\bf Theorem}
%\newtheorem{corollary}{\hspace{0pt}\bf Corollary}
\newtheorem{fact}{\hspace{0pt}\bf Fact}

\newcounter{remarkjs} \setcounter{remarkjs}{1}
\newenvironment{remarkjs}{ \vspace{-0.1cm} \noindent {\bf Remark
\theremarkjs :}
\addtocounter{remarkjs}{-1}\refstepcounter{remarkjs}\em } {
\addtocounter{remarkjs}{1} \vspace{-0.1cm} \normalfont }

%\newcounter{remarkjs} \setcounter{remarkjs}{1}
%\newenvironment{remarkjs}{\vspace{-0.1cm} \noindent {\bf Remark
%\theremarkjs :} \addtocounter{remarkjs}{-1} \refstepcounter{remarkjs}} { \vspace{-0.1cm} \normalfont \addtocounter{remarkjs}{1} }

\newtheorem{test}{\hspace{0pt}\it Test Case}
\newtheorem{definition}{\hspace{0pt}\bf Definition}
\newtheorem{example}{\hspace{0pt}\bf Example}

\def\proof      {\noindent\hspace{0pt}{\bf{Proof: }}}
\def\myQED      {\hfill$\blacksquare$\vspace{0.3cm}}





\def\bss{{\ensuremath{\boldsymbol{s}}}}
\def\bsz{{\ensuremath{\boldsymbol{z}}}}
\def\bsv{{\ensuremath{\boldsymbol{v}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%bar version
%capital alphabet
\def\bbarA{{\ensuremath{\bar A}}}
\def\bbarB{{\ensuremath{\bar B}}}
\def\bbarC{{\ensuremath{\bar C}}}
\def\bbarD{{\ensuremath{\bar D}}}
\def\bbarE{{\ensuremath{\bar E}}}
\def\bbarF{{\ensuremath{\bar F}}}
\def\bbarG{{\ensuremath{\bar G}}}
\def\bbarH{{\ensuremath{\bar H}}}
\def\bbarI{{\ensuremath{\bar I}}}
\def\bbarJ{{\ensuremath{\bar J}}}
\def\bbarK{{\ensuremath{\bar K}}}
\def\bbarL{{\ensuremath{\bar L}}}
\def\bbarM{{\ensuremath{\bar M}}}
\def\bbarN{{\ensuremath{\bar N}}}
\def\bbarO{{\ensuremath{\bar O}}}
\def\bbarP{{\ensuremath{\bar P}}}
\def\bbarQ{{\ensuremath{\bar Q}}}
\def\bbarR{{\ensuremath{\bar R}}}
\def\bbarW{{\ensuremath{\bar W}}}
\def\bbarU{{\ensuremath{\bar U}}}
\def\bbarV{{\ensuremath{\bar V}}}
\def\bbarS{{\ensuremath{\bar S}}}
\def\bbarT{{\ensuremath{\bar T}}}
\def\bbarX{{\ensuremath{\bar X}}}
\def\bbarY{{\ensuremath{\bar Y}}}
\def\bbarZ{{\ensuremath{\bar Z}}}
%lower case alphabet
\def\bbara{{\ensuremath{\bar a}}}
\def\bbarb{{\ensuremath{\bar b}}}
\def\bbarc{{\ensuremath{\bar c}}}
\def\bbard{{\ensuremath{\bar d}}}
\def\bbare{{\ensuremath{\bar e}}}
\def\bbarf{{\ensuremath{\bar f}}}
\def\bbarg{{\ensuremath{\bar g}}}
\def\bbarh{{\ensuremath{\bar h}}}
\def\bbari{{\ensuremath{\bar i}}}
\def\bbarj{{\ensuremath{\bar j}}}
\def\bbark{{\ensuremath{\bar k}}}
\def\bbarl{{\ensuremath{\bar l}}}
\def\bbarm{{\ensuremath{\bar m}}}
\def\bbarn{{\ensuremath{\bar n}}}
\def\bbaro{{\ensuremath{\bar o}}}
\def\bbarp{{\ensuremath{\bar p}}}
\def\bbarq{{\ensuremath{\bar q}}}
\def\bbarr{{\ensuremath{\bar r}}}
\def\bbarw{{\ensuremath{\bar w}}}
\def\bbaru{{\ensuremath{\bar u}}}
\def\bbarv{{\ensuremath{\bar v}}}
\def\bbars{{\ensuremath{\bar s}}}
\def\bbart{{\ensuremath{\bar t}}}
\def\bbarx{{\ensuremath{\bar x}}}
\def\bbary{{\ensuremath{\bar y}}}
\def\bbarz{{\ensuremath{\bar z}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of bar version
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%caligraph version
\def\ccalA{{\ensuremath{\mathcal A}}}
\def\ccalB{{\ensuremath{\mathcal B}}}
\def\ccalC{{\ensuremath{\mathcal C}}}
\def\ccalD{{\ensuremath{\mathcal D}}}
\def\ccalE{{\ensuremath{\mathcal E}}}
\def\ccalF{{\ensuremath{\mathcal F}}}
\def\ccalG{{\ensuremath{\mathcal G}}}
\def\ccalH{{\ensuremath{\mathcal H}}}
\def\ccalI{{\ensuremath{\mathcal I}}}
\def\ccalJ{{\ensuremath{\mathcal J}}}
\def\ccalK{{\ensuremath{\mathcal K}}}
\def\ccalL{{\ensuremath{\mathcal L}}}
\def\ccalM{{\ensuremath{\mathcal M}}}
\def\ccalN{{\ensuremath{\mathcal N}}}
\def\ccalO{{\ensuremath{\mathcal O}}}
\def\ccalP{{\ensuremath{\mathcal P}}}
\def\ccalQ{{\ensuremath{\mathcal Q}}}
\def\ccalR{{\ensuremath{\mathcal R}}}
\def\ccalW{{\ensuremath{\mathcal W}}}
\def\ccalU{{\ensuremath{\mathcal U}}}
\def\ccalV{{\ensuremath{\mathcal V}}}
\def\ccalS{{\ensuremath{\mathcal S}}}
\def\ccalT{{\ensuremath{\mathcal T}}}
\def\ccalX{{\ensuremath{\mathcal X}}}
\def\ccalY{{\ensuremath{\mathcal Y}}}
\def\ccalZ{{\ensuremath{\mathcal Z}}}
%lower case alphabet
\def\ccala{{\ensuremath{\mathcal a}}}
\def\ccalb{{\ensuremath{\mathcal b}}}
\def\ccalc{{\ensuremath{\mathcal c}}}
\def\ccald{{\ensuremath{\mathcal d}}}
\def\ccale{{\ensuremath{\mathcal e}}}
\def\ccalf{{\ensuremath{\mathcal f}}}
\def\ccalg{{\ensuremath{\mathcal g}}}
\def\ccalh{{\ensuremath{\mathcal h}}}
\def\ccali{{\ensuremath{\mathcal i}}}
\def\ccalj{{\ensuremath{\mathcal j}}}
\def\ccalk{{\ensuremath{\mathcal k}}}
\def\ccall{{\ensuremath{\mathcal l}}}
\def\ccalm{{\ensuremath{\mathcal m}}}
\def\ccaln{{\ensuremath{\mathcal n}}}
\def\ccalo{{\ensuremath{\mathcal o}}}
\def\ccalp{{\ensuremath{\mathcal p}}}
\def\ccalq{{\ensuremath{\mathcal q}}}
\def\ccalr{{\ensuremath{\mathcal r}}}
\def\ccalw{{\ensuremath{\mathcal w}}}
\def\ccalu{{\ensuremath{\mathcal u}}}
\def\ccalv{{\ensuremath{\mathcal v}}}
\def\ccals{{\ensuremath{\mathcal s}}}
\def\ccalt{{\ensuremath{\mathcal t}}}
\def\ccalx{{\ensuremath{\mathcal x}}}
\def\ccaly{{\ensuremath{\mathcal y}}}
\def\ccalz{{\ensuremath{\mathcal z}}}
\def\ccal0{{\ensuremath{\mathcal 0}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of caligraph version
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%hat version
%capital alphabet
\def\hhatA{{\ensuremath{\hat A}}}
\def\hhatB{{\ensuremath{\hat B}}}
\def\hhatC{{\ensuremath{\hat C}}}
\def\hhatD{{\ensuremath{\hat D}}}
\def\hhatE{{\ensuremath{\hat E}}}
\def\hhatF{{\ensuremath{\hat F}}}
\def\hhatG{{\ensuremath{\hat G}}}
\def\hhatH{{\ensuremath{\hat H}}}
\def\hhatI{{\ensuremath{\hat I}}}
\def\hhatJ{{\ensuremath{\hat J}}}
\def\hhatK{{\ensuremath{\hat K}}}
\def\hhatL{{\ensuremath{\hat L}}}
\def\hhatM{{\ensuremath{\hat M}}}
\def\hhatN{{\ensuremath{\hat N}}}
\def\hhatO{{\ensuremath{\hat O}}}
\def\hhatP{{\ensuremath{\hat P}}}
\def\hhatQ{{\ensuremath{\hat Q}}}
\def\hhatR{{\ensuremath{\hat R}}}
\def\hhatW{{\ensuremath{\hat W}}}
\def\hhatU{{\ensuremath{\hat U}}}
\def\hhatV{{\ensuremath{\hat V}}}
\def\hhatS{{\ensuremath{\hat S}}}
\def\hhatT{{\ensuremath{\hat T}}}
\def\hhatX{{\ensuremath{\hat X}}}
\def\hhatY{{\ensuremath{\hat Y}}}
\def\hhatZ{{\ensuremath{\hat Z}}}
%lower case alphabet
\def\hhata{{\ensuremath{\hat a}}}
\def\hhatb{{\ensuremath{\hat b}}}
\def\hhatc{{\ensuremath{\hat c}}}
\def\hhatd{{\ensuremath{\hat d}}}
\def\hhate{{\ensuremath{\hat e}}}
\def\hhatf{{\ensuremath{\hat f}}}
\def\hhatg{{\ensuremath{\hat g}}}
\def\hhath{{\ensuremath{\hat h}}}
\def\hhati{{\ensuremath{\hat i}}}
\def\hhatj{{\ensuremath{\hat j}}}
\def\hhatk{{\ensuremath{\hat k}}}
\def\hhatl{{\ensuremath{\hat l}}}
\def\hhatm{{\ensuremath{\hat m}}}
\def\hhatn{{\ensuremath{\hat n}}}
\def\hhato{{\ensuremath{\hat o}}}
\def\hhatp{{\ensuremath{\hat p}}}
\def\hhatq{{\ensuremath{\hat q}}}
\def\hhatr{{\ensuremath{\hat r}}}
\def\hhatw{{\ensuremath{\hat w}}}
\def\hhatu{{\ensuremath{\hat u}}}
\def\hhatv{{\ensuremath{\hat v}}}
\def\hhats{{\ensuremath{\hat s}}}
\def\hhatt{{\ensuremath{\hat t}}}
\def\hhatx{{\ensuremath{\hat x}}}
\def\hhaty{{\ensuremath{\hat y}}}
\def\hhatz{{\ensuremath{\hat z}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of hat version
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%tilde version
%capital alphabet
\def\tdA{{\ensuremath{\tilde A}}}
\def\tdB{{\ensuremath{\tilde B}}}
\def\tdC{{\ensuremath{\tilde C}}}
\def\tdD{{\ensuremath{\tilde D}}}
\def\tdE{{\ensuremath{\tilde E}}}
\def\tdF{{\ensuremath{\tilde F}}}
\def\tdG{{\ensuremath{\tilde G}}}
\def\tdH{{\ensuremath{\tilde H}}}
\def\tdI{{\ensuremath{\tilde I}}}
\def\tdJ{{\ensuremath{\tilde J}}}
\def\tdK{{\ensuremath{\tilde K}}}
\def\tdL{{\ensuremath{\tilde L}}}
\def\tdM{{\ensuremath{\tilde M}}}
\def\tdN{{\ensuremath{\tilde N}}}
\def\tdO{{\ensuremath{\tilde O}}}
\def\tdP{{\ensuremath{\tilde P}}}
\def\tdQ{{\ensuremath{\tilde Q}}}
\def\tdR{{\ensuremath{\tilde R}}}
\def\tdW{{\ensuremath{\tilde W}}}
\def\tdU{{\ensuremath{\tilde U}}}
\def\tdV{{\ensuremath{\tilde V}}}
\def\tdS{{\ensuremath{\tilde S}}}
\def\tdT{{\ensuremath{\tilde T}}}
\def\tdX{{\ensuremath{\tilde X}}}
\def\tdY{{\ensuremath{\tilde Y}}}
\def\tdZ{{\ensuremath{\tilde Z}}}
%lower case alphabet
\def\tda{{\ensuremath{\tilde a}}}
\def\tdb{{\ensuremath{\tilde b}}}
\def\tdc{{\ensuremath{\tilde c}}}
\def\tdd{{\ensuremath{\tilde d}}}
\def\tde{{\ensuremath{\tilde e}}}
\def\tdf{{\ensuremath{\tilde f}}}
\def\tdg{{\ensuremath{\tilde g}}}
\def\tdh{{\ensuremath{\tilde h}}}
\def\tdi{{\ensuremath{\tilde i}}}
\def\tdj{{\ensuremath{\tilde j}}}
\def\tdk{{\ensuremath{\tilde k}}}
\def\tdl{{\ensuremath{\tilde l}}}
\def\tdm{{\ensuremath{\tilde m}}}
\def\tdn{{\ensuremath{\tilde n}}}
\def\tdo{{\ensuremath{\tilde o}}}
\def\tdp{{\ensuremath{\tilde p}}}
\def\tdq{{\ensuremath{\tilde q}}}
\def\tdr{{\ensuremath{\tilde r}}}
\def\tdw{{\ensuremath{\tilde w}}}
\def\tdu{{\ensuremath{\tilde u}}}
\def\tdv{{\ensuremath{\tilde r}}}
\def\tds{{\ensuremath{\tilde s}}}
\def\tdt{{\ensuremath{\tilde t}}}
\def\tdx{{\ensuremath{\tilde x}}}
\def\tdy{{\ensuremath{\tilde y}}}
\def\tdz{{\ensuremath{\tilde z}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of tilde version
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%check version
%lower case alphabet
\def\chka{{\ensuremath{\check a}}}
\def\chkb{{\ensuremath{\check b}}}
\def\chkc{{\ensuremath{\check c}}}
\def\chkd{{\ensuremath{\check d}}}
\def\chke{{\ensuremath{\check e}}}
\def\chkf{{\ensuremath{\check f}}}
\def\chkg{{\ensuremath{\check g}}}
\def\chkh{{\ensuremath{\check h}}}
\def\chki{{\ensuremath{\check i}}}
\def\chkj{{\ensuremath{\check j}}}
\def\chkk{{\ensuremath{\check k}}}
\def\chkl{{\ensuremath{\check l}}}
\def\chkm{{\ensuremath{\check m}}}
\def\chkn{{\ensuremath{\check n}}}
\def\chko{{\ensuremath{\check o}}}
\def\chkp{{\ensuremath{\check p}}}
\def\chkq{{\ensuremath{\check q}}}
\def\chkr{{\ensuremath{\check r}}}
\def\chkw{{\ensuremath{\check w}}}
\def\chku{{\ensuremath{\check u}}}
\def\chkv{{\ensuremath{\check v}}}
\def\chks{{\ensuremath{\check s}}}
\def\chkt{{\ensuremath{\check t}}}
\def\chkx{{\ensuremath{\check x}}}
\def\chky{{\ensuremath{\check y}}}
\def\chkz{{\ensuremath{\check z}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of check version
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Bold version
% upper case bold
\def\bbA{{\ensuremath{\mathbf A}}}
\def\bbB{{\ensuremath{\mathbf B}}}
\def\bbC{{\ensuremath{\mathbf C}}}
\def\bbD{{\ensuremath{\mathbf D}}}
\def\bbE{{\ensuremath{\mathbf E}}}
\def\bbF{{\ensuremath{\mathbf F}}}
\def\bbG{{\ensuremath{\mathbf G}}}
\def\bbH{{\ensuremath{\mathbf H}}}
\def\bbI{{\ensuremath{\mathbf I}}}
\def\bbJ{{\ensuremath{\mathbf J}}}
\def\bbK{{\ensuremath{\mathbf K}}}
\def\bbL{{\ensuremath{\mathbf L}}}
\def\bbM{{\ensuremath{\mathbf M}}}
\def\bbN{{\ensuremath{\mathbf N}}}
\def\bbO{{\ensuremath{\mathbf O}}}
\def\bbP{{\ensuremath{\mathbf P}}}
\def\bbQ{{\ensuremath{\mathbf Q}}}
\def\bbR{{\ensuremath{\mathbf R}}}
\def\bbW{{\ensuremath{\mathbf W}}}
\def\bbU{{\ensuremath{\mathbf U}}}
\def\bbV{{\ensuremath{\mathbf V}}}
\def\bbS{{\ensuremath{\mathbf S}}}
\def\bbT{{\ensuremath{\mathbf T}}}
\def\bbX{{\ensuremath{\mathbf X}}}
\def\bbY{{\ensuremath{\mathbf Y}}}
\def\bbZ{{\ensuremath{\mathbf Z}}}
%lower case bold
\def\bba{{\ensuremath{\mathbf a}}}
\def\bbb{{\ensuremath{\mathbf b}}}
\def\bbc{{\ensuremath{\mathbf c}}}
\def\bbd{{\ensuremath{\mathbf d}}}
\def\bbe{{\ensuremath{\mathbf e}}}
\def\bbf{{\ensuremath{\mathbf f}}}
\def\bbg{{\ensuremath{\mathbf g}}}
\def\bbh{{\ensuremath{\mathbf h}}}
\def\bbi{{\ensuremath{\mathbf i}}}
\def\bbj{{\ensuremath{\mathbf j}}}
\def\bbk{{\ensuremath{\mathbf k}}}
\def\bbl{{\ensuremath{\mathbf l}}}
\def\bbm{{\ensuremath{\mathbf m}}}
\def\bbn{{\ensuremath{\mathbf n}}}
\def\bbo{{\ensuremath{\mathbf o}}}
\def\bbp{{\ensuremath{\mathbf p}}}
\def\bbq{{\ensuremath{\mathbf q}}}
\def\bbr{{\ensuremath{\mathbf r}}}
\def\bbw{{\ensuremath{\mathbf w}}}
\def\bbu{{\ensuremath{\mathbf u}}}
\def\bbv{{\ensuremath{\mathbf v}}}
\def\bbs{{\ensuremath{\mathbf s}}}
\def\bbt{{\ensuremath{\mathbf t}}}
\def\bbx{{\ensuremath{\mathbf x}}}
\def\bby{{\ensuremath{\mathbf y}}}
\def\bbz{{\ensuremath{\mathbf z}}}
\def\bb0{{\ensuremath{\mathbf 0}}}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%bar bold version
%upper case
%
\def\bbarbbA{{\bar{\ensuremath{\mathbf A}} }}
\def\bbarbbB{{\bar{\ensuremath{\mathbf B}} }}
\def\bbarbbC{{\bar{\ensuremath{\mathbf C}} }}
\def\bbarbbD{{\bar{\ensuremath{\mathbf D}} }}
\def\bbarbbE{{\bar{\ensuremath{\mathbf E}} }}
\def\bbarbbF{{\bar{\ensuremath{\mathbf F}} }}
\def\bbarbbG{{\bar{\ensuremath{\mathbf G}} }}
\def\bbarbbH{{\bar{\ensuremath{\mathbf H}} }}
\def\bbarbbI{{\bar{\ensuremath{\mathbf I}} }}
\def\bbarbbJ{{\bar{\ensuremath{\mathbf J}} }}
\def\bbarbbK{{\bar{\ensuremath{\mathbf K}} }}
\def\bbarbbL{{\bar{\ensuremath{\mathbf L}} }}
\def\bbarbbM{{\bar{\ensuremath{\mathbf M}} }}
\def\bbarbbN{{\bar{\ensuremath{\mathbf N}} }}
\def\bbarbbO{{\bar{\ensuremath{\mathbf O}} }}
\def\bbarbbP{{\bar{\ensuremath{\mathbf P}} }}
\def\bbarbbQ{{\bar{\ensuremath{\mathbf Q}} }}
\def\bbarbbR{{\bar{\ensuremath{\mathbf R}} }}
\def\bbarbbS{{\bar{\ensuremath{\mathbf S}} }}
\def\bbarbbT{{\bar{\ensuremath{\mathbf T}} }}
\def\bbarbbU{{\bar{\ensuremath{\mathbf U}} }}
\def\bbarbbV{{\bar{\ensuremath{\mathbf V}} }}
\def\bbarbbW{{\bar{\ensuremath{\mathbf W}} }}
\def\bbarbbX{{\bar{\ensuremath{\mathbf X}} }}
\def\bbarbbY{{\bar{\ensuremath{\mathbf Y}} }}
\def\bbarbbZ{{\bar{\ensuremath{\mathbf Z}} }}
%
%lower case
%
\def\bbarbba{{\bar{\ensuremath{\mathbf a}} }}
\def\bbarbbb{{\bar{\ensuremath{\mathbf b}} }}
\def\bbarbbc{{\bar{\ensuremath{\mathbf c}} }}
\def\bbarbbd{{\bar{\ensuremath{\mathbf d}} }}
\def\bbarbbe{{\bar{\ensuremath{\mathbf e}} }}
\def\bbarbbf{{\bar{\ensuremath{\mathbf f}} }}
\def\bbarbbg{{\bar{\ensuremath{\mathbf g}} }}
\def\bbarbbh{{\bar{\ensuremath{\mathbf h}} }}
\def\bbarbbi{{\bar{\ensuremath{\mathbf i}} }}
\def\bbarbbj{{\bar{\ensuremath{\mathbf j}} }}
\def\bbarbbk{{\bar{\ensuremath{\mathbf k}} }}
\def\bbarbbl{{\bar{\ensuremath{\mathbf l}} }}
\def\bbarbbm{{\bar{\ensuremath{\mathbf m}} }}
\def\bbarbbn{{\bar{\ensuremath{\mathbf n}} }}
\def\bbarbbo{{\bar{\ensuremath{\mathbf o}} }}
\def\bbarbbp{{\bar{\ensuremath{\mathbf p}} }}
\def\bbarbbq{{\bar{\ensuremath{\mathbf q}} }}
\def\bbarbbr{{\bar{\ensuremath{\mathbf r}} }}
\def\bbarbbs{{\bar{\ensuremath{\mathbf s}} }}
\def\bbarbbt{{\bar{\ensuremath{\mathbf t}} }}
\def\bbarbbu{{\bar{\ensuremath{\mathbf u}} }}
\def\bbarbbv{{\bar{\ensuremath{\mathbf v}} }}
\def\bbarbbw{{\bar{\ensuremath{\mathbf w}} }}
\def\bbarbbx{{\bar{\ensuremath{\mathbf x}} }}
\def\bbarbby{{\bar{\ensuremath{\mathbf y}} }}
\def\bbarbbz{{\bar{\ensuremath{\mathbf z}} }}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of bar bold bersion
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%hat bold version
%upper case
%
\def\hhatbbA{{\hat{\ensuremath{\mathbf A}} }}
\def\hhatbbB{{\hat{\ensuremath{\mathbf B}} }}
\def\hhatbbC{{\hat{\ensuremath{\mathbf C}} }}
\def\hhatbbD{{\hat{\ensuremath{\mathbf D}} }}
\def\hhatbbE{{\hat{\ensuremath{\mathbf E}} }}
\def\hhatbbF{{\hat{\ensuremath{\mathbf F}} }}
\def\hhatbbG{{\hat{\ensuremath{\mathbf G}} }}
\def\hhatbbH{{\hat{\ensuremath{\mathbf H}} }}
\def\hhatbbI{{\hat{\ensuremath{\mathbf I}} }}
\def\hhatbbJ{{\hat{\ensuremath{\mathbf J}} }}
\def\hhatbbK{{\hat{\ensuremath{\mathbf K}} }}
\def\hhatbbL{{\hat{\ensuremath{\mathbf L}} }}
\def\hhatbbM{{\hat{\ensuremath{\mathbf M}} }}
\def\hhatbbN{{\hat{\ensuremath{\mathbf N}} }}
\def\hhatbbO{{\hat{\ensuremath{\mathbf O}} }}
\def\hhatbbP{{\hat{\ensuremath{\mathbf P}} }}
\def\hhatbbQ{{\hat{\ensuremath{\mathbf Q}} }}
\def\hhatbbR{{\hat{\ensuremath{\mathbf R}} }}
\def\hhatbbS{{\hat{\ensuremath{\mathbf S}} }}
\def\hhatbbT{{\hat{\ensuremath{\mathbf T}} }}
\def\hhatbbU{{\hat{\ensuremath{\mathbf U}} }}
\def\hhatbbV{{\hat{\ensuremath{\mathbf V}} }}
\def\hhatbbW{{\hat{\ensuremath{\mathbf W}} }}
\def\hhatbbX{{\hat{\ensuremath{\mathbf X}} }}
\def\hhatbbY{{\hat{\ensuremath{\mathbf Y}} }}
\def\hhatbbZ{{\hat{\ensuremath{\mathbf Z}} }}
%
%lower case
%
\def\hhatbba{{\hat{\ensuremath{\mathbf a}} }}
\def\hhatbbb{{\hat{\ensuremath{\mathbf b}} }}
\def\hhatbbc{{\hat{\ensuremath{\mathbf c}} }}
\def\hhatbbd{{\hat{\ensuremath{\mathbf d}} }}
\def\hhatbbe{{\hat{\ensuremath{\mathbf e}} }}
\def\hhatbbf{{\hat{\ensuremath{\mathbf f}} }}
\def\hhatbbg{{\hat{\ensuremath{\mathbf g}} }}
\def\hhatbbh{{\hat{\ensuremath{\mathbf h}} }}
\def\hhatbbi{{\hat{\ensuremath{\mathbf i}} }}
\def\hhatbbj{{\hat{\ensuremath{\mathbf j}} }}
\def\hhatbbk{{\hat{\ensuremath{\mathbf k}} }}
\def\hhatbbl{{\hat{\ensuremath{\mathbf l}} }}
\def\hhatbbm{{\hat{\ensuremath{\mathbf m}} }}
\def\hhatbbn{{\hat{\ensuremath{\mathbf n}} }}
\def\hhatbbo{{\hat{\ensuremath{\mathbf o}} }}
\def\hhatbbp{{\hat{\ensuremath{\mathbf p}} }}
\def\hhatbbq{{\hat{\ensuremath{\mathbf q}} }}
\def\hhatbbr{{\hat{\ensuremath{\mathbf r}} }}
\def\hhatbbs{{\hat{\ensuremath{\mathbf s}} }}
\def\hhatbbt{{\hat{\ensuremath{\mathbf t}} }}
\def\hhatbbu{{\hat{\ensuremath{\mathbf u}} }}
\def\hhatbbv{{\hat{\ensuremath{\mathbf v}} }}
\def\hhatbbw{{\hat{\ensuremath{\mathbf w}} }}
\def\hhatbbx{{\hat{\ensuremath{\mathbf x}} }}
\def\hhatbby{{\hat{\ensuremath{\mathbf y}} }}
\def\hhatbbz{{\hat{\ensuremath{\mathbf z}} }}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of hat bold  bersion
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%tilde bold version
%upper case
%
\def\tdbbA{{\tilde{\ensuremath{\mathbf A}} }}
\def\tdbbB{{\tilde{\ensuremath{\mathbf B}} }}
\def\tdbbC{{\tilde{\ensuremath{\mathbf C}} }}
\def\tdbbD{{\tilde{\ensuremath{\mathbf D}} }}
\def\tdbbE{{\tilde{\ensuremath{\mathbf E}} }}
\def\tdbbF{{\tilde{\ensuremath{\mathbf F}} }}
\def\tdbbG{{\tilde{\ensuremath{\mathbf G}} }}
\def\tdbbH{{\tilde{\ensuremath{\mathbf H}} }}
\def\tdbbI{{\tilde{\ensuremath{\mathbf I}} }}
\def\tdbbJ{{\tilde{\ensuremath{\mathbf J}} }}
\def\tdbbK{{\tilde{\ensuremath{\mathbf K}} }}
\def\tdbbL{{\tilde{\ensuremath{\mathbf L}} }}
\def\tdbbM{{\tilde{\ensuremath{\mathbf M}} }}
\def\tdbbN{{\tilde{\ensuremath{\mathbf N}} }}
\def\tdbbO{{\tilde{\ensuremath{\mathbf O}} }}
\def\tdbbP{{\tilde{\ensuremath{\mathbf P}} }}
\def\tdbbQ{{\tilde{\ensuremath{\mathbf Q}} }}
\def\tdbbR{{\tilde{\ensuremath{\mathbf R}} }}
\def\tdbbS{{\tilde{\ensuremath{\mathbf S}} }}
\def\tdbbT{{\tilde{\ensuremath{\mathbf T}} }}
\def\tdbbU{{\tilde{\ensuremath{\mathbf U}} }}
\def\tdbbV{{\tilde{\ensuremath{\mathbf V}} }}
\def\tdbbW{{\tilde{\ensuremath{\mathbf W}} }}
\def\tdbbX{{\tilde{\ensuremath{\mathbf X}} }}
\def\tdbbY{{\tilde{\ensuremath{\mathbf Y}} }}
\def\tdbbZ{{\tilde{\ensuremath{\mathbf Z}} }}
%
%lower case
%
\def\tdbba{{\tilde{\ensuremath{\mathbf a}} }}
\def\tdbbb{{\tilde{\ensuremath{\mathbf b}} }}
\def\tdbbc{{\tilde{\ensuremath{\mathbf c}} }}
\def\tdbbd{{\tilde{\ensuremath{\mathbf d}} }}
\def\tdbbe{{\tilde{\ensuremath{\mathbf e}} }}
\def\tdbbf{{\tilde{\ensuremath{\mathbf f}} }}
\def\tdbbg{{\tilde{\ensuremath{\mathbf g}} }}
\def\tdbbh{{\tilde{\ensuremath{\mathbf h}} }}
\def\tdbbi{{\tilde{\ensuremath{\mathbf i}} }}
\def\tdbbj{{\tilde{\ensuremath{\mathbf j}} }}
\def\tdbbk{{\tilde{\ensuremath{\mathbf k}} }}
\def\tdbbl{{\tilde{\ensuremath{\mathbf l}} }}
\def\tdbbm{{\tilde{\ensuremath{\mathbf m}} }}
\def\tdbbn{{\tilde{\ensuremath{\mathbf n}} }}
\def\tdbbo{{\tilde{\ensuremath{\mathbf o}} }}
\def\tdbbp{{\tilde{\ensuremath{\mathbf p}} }}
\def\tdbbq{{\tilde{\ensuremath{\mathbf q}} }}
\def\tdbbr{{\tilde{\ensuremath{\mathbf r}} }}
\def\tdbbs{{\tilde{\ensuremath{\mathbf s}} }}
\def\tdbbt{{\tilde{\ensuremath{\mathbf t}} }}
\def\tdbbu{{\tilde{\ensuremath{\mathbf u}} }}
\def\tdbbv{{\tilde{\ensuremath{\mathbf v}} }}
\def\tdbbw{{\tilde{\ensuremath{\mathbf w}} }}
\def\tdbbx{{\tilde{\ensuremath{\mathbf x}} }}
\def\tdbby{{\tilde{\ensuremath{\mathbf y}} }}
\def\tdbbz{{\tilde{\ensuremath{\mathbf z}} }}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of tilde bold  bersion
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%bold caligraph
%
\def\bbcalA{\mbox{\boldmath $\mathcal{A}$}}
\def\bbcalB{\mbox{\boldmath $\mathcal{B}$}}
\def\bbcalC{\mbox{\boldmath $\mathcal{C}$}}
\def\bbcalD{\mbox{\boldmath $\mathcal{D}$}}
\def\bbcalE{\mbox{\boldmath $\mathcal{E}$}}
\def\bbcalF{\mbox{\boldmath $\mathcal{F}$}}
\def\bbcalG{\mbox{\boldmath $\mathcal{G}$}}
\def\bbcalH{\mbox{\boldmath $\mathcal{H}$}}
\def\bbcalI{\mbox{\boldmath $\mathcal{I}$}}
\def\bbcalJ{\mbox{\boldmath $\mathcal{J}$}}
\def\bbcalK{\mbox{\boldmath $\mathcal{K}$}}
\def\bbcalL{\mbox{\boldmath $\mathcal{L}$}}
\def\bbcalM{\mbox{\boldmath $\mathcal{M}$}}
\def\bbcalN{\mbox{\boldmath $\mathcal{N}$}}
\def\bbcalO{\mbox{\boldmath $\mathcal{O}$}}
\def\bbcalP{\mbox{\boldmath $\mathcal{P}$}}
\def\bbcalQ{\mbox{\boldmath $\mathcal{Q}$}}
\def\bbcalR{\mbox{\boldmath $\mathcal{R}$}}
\def\bbcalW{\mbox{\boldmath $\mathcal{W}$}}
\def\bbcalU{\mbox{\boldmath $\mathcal{U}$}}
\def\bbcalV{\mbox{\boldmath $\mathcal{V}$}}
\def\bbcalS{\mbox{\boldmath $\mathcal{S}$}}
\def\bbcalT{\mbox{\boldmath $\mathcal{T}$}}
\def\bbcalX{\mbox{\boldmath $\mathcal{X}$}}
\def\bbcalY{\mbox{\boldmath $\mathcal{Y}$}}
\def\bbcalZ{\mbox{\boldmath $\mathcal{Z}$}}
%
\def\bbcale{\mbox{\boldmath $\mathcal{e}$}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of caligraph
%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%tilde Greek
%
\def\tdupsilon{\tilde\upsilon}
\def\tdalpha{\tilde\alpha}
\def\tdbeta{\tilde\beta}
\def\tdgamma{\tilde\gamma}
\def\tddelta{\tilde\delta}
\def\tdepsilon{\tilde\epsilon}
\def\tdvarepsilon{\tilde\varepsilon}
\def\tdzeta{\tilde\zeta}
\def\tdeta{\tilde\eta}
\def\tdtheta{\tilde\theta}
\def\tdvartheta{\tilde\vartheta}

\def\tdiota{\tilde\iota}
\def\tdkappa{\tilde\kappa}
\def\tdlambda{\tilde\lambda}
\def\tdmu{\tilde\mu}
\def\tdnu{\tilde\nu}
\def\tdxi{\tilde\xi}
\def\tdpi{\tilde\pi}
\def\tdrho{\tilde\rho}
\def\tdvarrho{\tilde\varrho}
\def\tdsigma{\tilde\sigma}
\def\tdvarsigma{\tilde\varsigma}
\def\tdtau{\tilde\tau}
\def\tdupsilon{\tilde\upsilon}
\def\tdphi{\tilde\phi}
\def\tdvarphi{\tilde\varphi}
\def\tdchi{\tilde\chi}
\def\tdpsi{\tilde\psi}
\def\tdomega{\tilde\omega}

\def\tdGamma{\tilde\Gamma}
\def\tdDelta{\tilde\Delta}
\def\tdTheta{\tilde\Theta}
\def\tdLambda{\tilde\Lambda}
\def\tdXi{\tilde\Xi}
\def\tdPi{\tilde\Pi}
\def\tdSigma{\tilde\Sigma}
\def\tdUpsilon{\tilde\Upsilon}
\def\tdPhi{\tilde\Phi}
\def\tdPsi{\tilde\Psi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of title  Greek
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%bar Greek
%
\def\bbarupsilon{\bar\upsilon}
\def\bbaralpha{\bar\alpha}
\def\bbarbeta{\bar\beta}
\def\bbargamma{\bar\gamma}
\def\bbarsigma{\bar\sigma}
\def\bbardelta{\bar\delta}
\def\bbarepsilon{\bar\epsilon}
\def\bbarvarepsilon{\bar\varepsilon}
\def\bbarzeta{\bar\zeta}
\def\bbareta{\bar\eta}
\def\bbartheta{\bar\theta}
\def\bbarvartheta{\bar\vartheta}

\def\bbariota{\bar\iota}
\def\bbarkappa{\bar\kappa}
\def\bbarlambda{\bar\lambda}
\def\bbarmu{\bar\mu}
\def\bbarnu{\bar\nu}
\def\bbarxi{\bar\xi}
\def\bbarpi{\bar\pi}
\def\bbarrho{\bar\rho}
\def\bbarvarrho{\bar\varrho}
\def\bbarvarsigma{\bar\varsigma}
\def\bbarphi{\bar\phi}
\def\bbarvarphi{\bar\varphi}
\def\bbarchi{\bar\chi}
\def\bbarpsi{\bar\psi}
\def\bbaromega{\bar\omega}

\def\bbarGamma{\bar\Gamma}
\def\bbarDelta{\bar\Delta}
\def\bbarTheta{\bar\Theta}
\def\bbarLambda{\bar\Lambda}
\def\bbarXi{\bar\Xi}
\def\bbarPi{\bar\Pi}
\def\bbarSigma{\bar\Sigma}
\def\bbarUpsilon{\bar\Upsilon}
\def\bbarPhi{\bar\Phi}
\def\bbarPsi{\bar\Psi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of bar  Greek
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%begion of check Greek
%
\def\chkupsilon{\check\upsilon}
\def\chkalpha{\check\alpha}
\def\chkbeta{\check\beta}
\def\chkgamma{\check\gamma}
\def\chkdelta{\check\delta}
\def\chkepsilon{\check\epsilon}
\def\chkvarepsilon{\check\varepsilon}
\def\chkzeta{\check\zeta}
\def\chketa{\check\eta}
\def\chktheta{\check\theta}
\def\chkvartheta{\check\vartheta}

\def\chkiota{\check\iota}
\def\chkkappa{\check\kappa}
\def\chklambda{\check\lambda}
\def\chkmu{\check\mu}
\def\chknu{\check\nu}
\def\chkxi{\check\xi}
\def\chkpi{\check\pi}
\def\chkrho{\check\rho}
\def\chkvarrho{\check\varrho}
\def\chksigma{\check\sigma}
\def\chkvarsigma{\check\varsigma}
\def\chktau{\check\tau}
\def\chkupsilon{\check\upsilon}
\def\chkphi{\check\phi}
\def\chkvarphi{\check\varphi}
\def\chkchi{\check\chi}
\def\chkpsi{\check\psi}
\def\chkomega{\check\omega}

\def\chkGamma{\check\Gamma}
\def\chkDelta{\check\Delta}
\def\chkTheta{\check\Theta}
\def\chkLambda{\check\Lambda}
\def\chkXi{\check\Xi}
\def\chkPi{\check\Pi}
\def\chkSigma{\check\Sigma}
\def\chkUpsilon{\check\Upsilon}
\def\chkPhi{\check\Phi}
\def\chkPsi{\check\Psi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of check Greek
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Bold Greek letter
%
\def\bbupsilon{{\mbox{\boldmath $\upsilon$}}}
\def\bbalpha{{\mbox{\boldmath $\alpha$}}}
\def\bbbeta{{\mbox{\boldmath $\beta$}}}
\def\bbgamma{{\mbox{\boldmath $\gamma$}}}
\def\bbdelta{{\mbox{\boldmath $\delta$}}}
\def\bbepsilon{{\mbox{\boldmath $\epsilon$}}}
\def\bbvarepsilon{{\mbox{\boldmath $\varepsilon$}}}
\def\bbzeta{{\mbox{\boldmath $\zeta$}}}
\def\bbeta{{\mbox{\boldmath $\eta$}}}
\def\bbtheta{{\mbox{\boldmath $\theta$}}}
\def\bbvartheta{{\mbox{\boldmath $\vartheta$}}}

\def\bbiota{{\mbox{\boldmath $\iota$}}}
\def\bbkappa{{\mbox{\boldmath $\kappa$}}}
\def\bblambda{{\mbox{\boldmath $\lambda$}}}
\def\bbmu{{\mbox{\boldmath $\mu$}}}
\def\bbnu{{\mbox{\boldmath $\nu$}}}
\def\bbxi{{\mbox{\boldmath $\xi$}}}
\def\bbpi{{\mbox{\boldmath $\pi$}}}
\def\bbrho{{\mbox{\boldmath $\rho$}}}
\def\bbvarrho{{\mbox{\boldmath $\varrho$}}}
\def\bbvarsigma{{\mbox{\boldmath $\varsigma$}}}
\def\bbphi{{\mbox{\boldmath $\phi$}}}
\def\bbvarphi{{\mbox{\boldmath $\varphi$}}}
\def\bbchi{{\mbox{\boldmath $\chi$}}}
\def\bbpsi{{\mbox{\boldmath $\psi$}}}
\def\bbomega{{\mbox{\boldmath $\omega$}}}

\def\bbGamma{{\mbox{\boldmath $\Gamma$}}}
\def\bbDelta{{\mbox{\boldmath $\Delta$}}}
\def\bbTheta{{\mbox{\boldmath $\Theta$}}}
\def\bbLambda{{\mbox{\boldmath $\Lambda$}}}
\def\bbXi{{\mbox{\boldmath $\Xi$}}}
\def\bbPi{{\mbox{\boldmath $\Pi$}}}
\def\bbSigma{{\mbox{\boldmath $\Sigma$}}}
\def\bbUpsilon{{\mbox{\boldmath $\Upsilon$}}}
\def\bbPhi{{\mbox{\boldmath $\Phi$}}}
\def\bbPsi{{\mbox{\boldmath $\Psi$}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of Bold Greek
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%bar Bold Greek
%
\def\bbarbbupsilon{\bar\bbupsilon}
\def\bbarbbalpha{\bar\bbalpha}
\def\bbarbbbeta{\bar\bbbeta}
\def\bbarbbgamma{\bar\bbgamma}
\def\bbarbbdelta{\bar\bbdelta}
\def\bbarbbepsilon{\bar\bbepsilon}
\def\bbarbbvarepsilon{\bar\bbvarepsilon}
\def\bbarbbzeta{\bar\bbzeta}
\def\bbarbbeta{\bar\bbeta}
\def\bbarbbtheta{\bar\bbtheta}
\def\bbarbbvartheta{\bar\bbvartheta}

\def\bbarbbiota{\bar\bbiota}
\def\bbarbbkappa{\bar\bbkappa}
\def\bbarbblambda{\bar\bblambda}
\def\bbarbbmu{\bar\bbmu}
\def\bbarbbnu{\bar\bbnu}
\def\bbarbbxi{\bar\bbxi}
\def\bbarbbpi{\bar\bbpi}
\def\bbarbbrho{\bar\bbrho}
\def\bbarbbvarrho{\bar\bbvarrho}
\def\bbarbbvarsigma{\bar\bbvarsigma}
\def\bbarbbphi{\bar\bbphi}
\def\bbarbbvarphi{\bar\bbvarphi}
\def\bbarbbchi{\bar\bbchi}
\def\bbarbbpsi{\bar\bbpsi}
\def\bbarbbomega{\bar\bbomega}

\def\bbarbbGamma{\bar\bbGamma}
\def\bbarbbDelta{\bar\bbDelta}
\def\bbarbbTheta{\bar\bbTheta}
\def\bbarbbLambda{\bar\bbLambda}
\def\bbarbbXi{\bar\bbXi}
\def\bbarbbPi{\bar\bbPi}
\def\bbarbbSigma{\bar\bbSigma}
\def\bbarbbUpsilon{\bar\bbUpsilon}
\def\bbarbbPhi{\bar\bbPhi}
\def\bbarbbPsi{\bar\bbPsi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of bar Bold Greek
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%hat Bold Greek
%
\def\hhatbbupsilon{\hat\bbupsilon}
\def\hhatbbalpha{\hat\bbalpha}
\def\hhatbbbeta{\hat\bbbeta}
\def\hhatbbgamma{\hat\bbgamma}
\def\hhatbbdelta{\hat\bbdelta}
\def\hhatbbepsilon{\hat\bbepsilon}
\def\hhatbbvarepsilon{\hat\bbvarepsilon}
\def\hhatbbzeta{\hat\bbzeta}
\def\hhatbbeta{\hat\bbeta}
\def\hhatbbtheta{\hat\bbtheta}
\def\hhatbbvartheta{\hat\bbvartheta}

\def\hhatbbiota{\hat\bbiota}
\def\hhatbbkappa{\hat\bbkappa}
\def\hhatbblambda{\hat\bblambda}
\def\hhatbbmu{\hat\bbmu}
\def\hhatbbnu{\hat\bbnu}
\def\hhatbbxi{\hat\bbxi}
\def\hhatbbpi{\hat\bbpi}
\def\hhatbbrho{\hat\bbrho}
\def\hhatbbvarrho{\hat\bbvarrho}
\def\hhatbbvarsigma{\hat\bbvarsigma}
\def\hhatbbphi{\hat\bbphi}
\def\hhatbbvarphi{\hat\bbvarphi}
\def\hhatbbchi{\hat\bbchi}
\def\hhatbbpsi{\hat\bbpsi}
\def\hhatbbomega{\hat\bbomega}

\def\hhatbbGamma{\hat\bbGamma}
\def\hhatbbDelta{\hat\bbDelta}
\def\hhatbbTheta{\hat\bbTheta}
\def\hhatbbLambda{\hat\bbLambda}
\def\hhatbbXi{\hat\bbXi}
\def\hhatbbPi{\hat\bbPi}
\def\hhatbbSigma{\hat\bbSigma}
\def\hhatbbUpsilon{\hat\bbUpsilon}
\def\hhatbbPhi{\hat\bbPhi}
\def\hhatbbPsi{\hat\bbPsi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of hat Bold Greek
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%tilde Bold Greek
%
\def\tdbbupsilon{\tilde\bbupsilon}
\def\tdbbalpha{\tilde\bbalpha}
\def\tdbbbeta{\tilde\bbbeta}
\def\tdbbgamma{\tilde\bbgamma}
\def\tdbbdelta{\tilde\bbdelta}
\def\tdbbepsilon{\tilde\bbepsilon}
\def\tdbbvarepsilon{\tilde\bbvarepsilon}
\def\tdbbzeta{\tilde\bbzeta}
\def\tdbbeta{\tilde\bbeta}
\def\tdbbtheta{\tilde\bbtheta}
\def\tdbbvartheta{\tilde\bbvartheta}

\def\tdbbiota{\tilde\bbiota}
\def\tdbbkappa{\tilde\bbkappa}
\def\tdbblambda{\tilde\bblambda}
\def\tdbbmu{\tilde\bbmu}
\def\tdbbnu{\tilde\bbnu}
\def\tdbbxi{\tilde\bbxi}
\def\tdbbpi{\tilde\bbpi}
\def\tdbbrho{\tilde\bbrho}
\def\tdbbvarrho{\tilde\bbvarrho}
\def\tdbbvarsigma{\tilde\bbvarsigma}
\def\tdbbphi{\tilde\bbphi}
\def\tdbbvarphi{\tilde\bbvarphi}
\def\tdbbchi{\tilde\bbchi}
\def\tdbbpsi{\tilde\bbpsi}
\def\tdbbomega{\tilde\bbomega}

\def\tdbbGamma{\tilde\bbGamma}
\def\tdbbDelta{\tilde\bbDelta}
\def\tdbbTheta{\tilde\bbTheta}
\def\tdbbLambda{\tilde\bbLambda}
\def\tdbbXi{\tilde\bbXi}
\def\tdbbPi{\tilde\bbPi}
\def\tdbbSigma{\tilde\bbSigma}
\def\tdbbUpsilon{\tilde\bbUpsilon}
\def\tdbbPhi{\tilde\bbPhi}
\def\tdbbPsi{\tilde\bbPsi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of tilde Bold Greek
\def\deltat{\triangle t}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%hat greek
%
\def\hhattheta{\hat\theta}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%end of hat greek
%
%
%
%
\def\var{{\rm var}}
\def\bbtau{{\mbox{\boldmath $\tau$}}}
%
%
%
%
%
%misc
%\def\diag{{\text{diag}}}
%\def\tr{{\text{tr}}}
%\def\tdbbs{{\tilde{\bfs}}}
%\def\tdbby{{\tilde{\bfy}}}
%\def\rank{{\text{rank}}}
%\def\bbarbbs{{\bar{\bfs}}}
%\def\bbarbbH{{\bar{\bfH}}}
%\def\bbarbby{{\bar{\bfy}}}
%\def\tdbbH{{\tilde \bfH}}
%\def\tdbbh{{\tilde \bfh}}
%\def\tdbbeta{{\tilde \bfeta}}
%\def\checkbby{{\check\bfy}}
%\def\checkbbs{{\check\bfs}}
%\def\checkbbx{{\check\bfx}}
%\def\checkbbeta{{\check\bfeta}}
%\def\checktdbbs{{\check\tdbbs}}

